Cyclotomic synthetic spectra

We define an $\infty$-category $\mathrm{CycSyn}$ of $p$-typical cyclotomic synthetic spectra and prove that the motivic filtration on $\mathrm{THH}(R;\mathbf{Z}_p)$, defined by Bhatt, Morrow, and Scholze when $R$ is quasisyntomic and by Hahn, Raksit, and Wilson in the chromatically quasisyntomic case, naturally admits the structure of a $p$-typical cyclotomic synthetic spectrum. As a consequence, we obtain new bounds on the syntomic cohomology of connective chromatically quasisyntomic $\mathbf{E}_\infty$-ring spectra.

==> theorem_A.tex <==
\section{Proof of Theorem E}\label{sec:thm_a}

%\subsection{Comparison to prismatic F-Gauges}

%The (Nygaard complete) prismatic cohomology of a $p$-complete ring was originally defined in terms of filtrations on topological Hochschild homology and related invariants by Bhatt, Morrow, and Scholze in \cite{bms2}. These filtrations agree with those we have studied in this paper by \cite[Theorem 5.0.3]{hrw} and Lemma~\ref{lem: even filtration comparison general}. As such one should expect there to be a connection between modules over $F^{\geq \star}_\ev\THH(R;\bZ_p)$ and quasicoherent sheaves on $\mathrm{Spf}(R)^{\mathrm{syn}}$. In this subsection we discuss the relationship.

%\begin{notation}
 %   Let $\F^{\geq \star}_\ev\THH(\mathcal{O}; \bZ_p)$ denote the functor from quasisyntomic rings to $\CycSyn_p$ given by $R\mapsto\F^{\geq \star}_\ev\THH(R;\bZ_p)$.
 %   By \cite[Theorem 5.0.3]{hrw}, this is a quasisyntomic sheaf and so we will consider it as such moving forward.

 %   Let $\CycSyn_{\F^{\geq \star}_\ev\THH(\mathcal{O};\bZ_p)}$ denote the $\infty$-category of
 %   modules over $\F^{\geq \star}_{\ev}\THH(\mathcal{O};\bZ_p)$
   % in $\mathrm{Shv}_{\mathrm{QSyn}}(\CycSyn)$.
%\end{notation}

%\begin{remark}
%    Because of set-theoretic issues we do not have a sheafification functor for the quasisyntomic
 %   topology, and so in particular the usual construction of the symmetric monoidal structure on
 %   the category of sheaves does not go through. Nevertheless, $\F^{\geq
    %\star}_{\ev}\THH(\mathcal{O};\bZ_p)$ is an $\bE_\infty$ ring in the category of presheaves, and
 %   so we can define the category of modules to be the pullback
%    \[
 %   \begin{tikzcd}
  %  \CycSyn_{F^{\geq \star}_{\ev}\THH(\mathcal{O};\bZ_p)} \ar[d] \ar[r] & \mathrm{Shv}_{\mathrm{QSyn}}(\CycSyn)\ar[d]\\
 %   \mathrm{Fun}(\mathrm{QSyn}, \CycSyn)_{F^{^\geq *}_{\ev}\THH(\mathcal{O};\bZ_p)} \ar[r] & \mathrm{Fun}(\mathrm{QSyn}, \CycSyn)
%    \end{tikzcd}
%    \] in $\widehat{\mathrm{Cat}}_\infty^{ex}$.
%\end{remark}

%\begin{variant}
 %   Let $R$ be a quasisyntomic ring.
%    Then we can make relative versions $\F^{\geq
    %\star}_\ev\THH(\mathcal{O}_R;\bZ_p):\mathrm{qSyn}_R\to \CycSyn$ and $\CycSyn_{\F^{\geq
    %\star}_\ev\THH(\mathcal{O}_R;\bZ_p)}$. Note that there are natural restriction functors
   % \[\CycSyn_{\F^{\geq \star}_\ev\THH(\mathcal{O};\bZ_p)}\to \CycSyn_{\F^{\geq
    %\star}_\ev\THH(\mathcal{O}_R;\bZ_p)}\] and \[\CycSyn_{\F^{\geq
    %\star}_\ev\THH(\mathcal{O}_S;\bZ_p)}\to \CycSyn_{\F^{\geq \star}_\ev\THH(\mathcal{O}_R;\bZ_p)}\]
   % when $R\to S$ is quasisyntomic which we will denote by $\F^{\geq \star}\mathcal{M}\mapsto
    %\F^{\geq \star}\mathcal{M}|_R$.
%\end{variant}

%\begin{lemma}
 %   There is a cartesian square 
 %   \[
 %   \begin{tikzcd}
%    \CycSyn_{\F^{\geq \star}_\ev\THH(\mathcal{O};\bZ_p)} \ar[d] \ar[r] & \mathrm{Shv}_{\mathrm{QRSP}}(\CycSyn)\ar[d]\\
%    \mathrm{Fun}(\mathrm{QRSP}, \CycSyn)_{\F^{\geq \star}_\ev\THH(\mathcal{O};\bZ_p)} \ar[r] & \mathrm{Fun}(\mathrm{QRSP}, \CycSyn)
 %   \end{tikzcd}
 %   \] in $\widehat{\mathrm{Cat}}^{ex}_\infty$. The analogous squares for the variants also hold.
%\end{lemma}

%\begin{proof}
 %For any fixed Grothendieck universe this follows from Barr--Beck--Lurie and the unfolding
%    equivalence of \cite[Prop.~4.31]{bms2}.
 %   Since the functor inducing these equivalences does not depend on the choice of Grothendieck universe the result then follows.
%\end{proof}

%\begin{lemma}
 %   Let $R$ be a perfectoid ring and $A$ a formally smooth $R$-algebra.
%    Then the global sections functor \[\CycSyn_{\F^{\geq \star}_\ev\THH(\mathcal{O}_A;\bZ_p)}\to
 %   \CycSyn_{\F^{\geq \star}_\ev\THH(A;\bZ_p)}\] admits a fully faithful left adjoint on bounded below objects.
%\end{lemma}

%\begin{proof}
 %   For $\F^{\geq \star}M\in \CycSyn_{\F^{\geq \star}_\ev\THH(A;\bZ_p)}$, let $\underline{\F^{\geq \star}M}\in \mathrm{Fun}(\mathrm{QSyn}_{A}, \CycSyn)$
%    denote the associated constant presheaf.
 %   We can then construct a presheaf $\F^{\geq \star}\mathcal{M}$ by taking \[\F^{\geq
 %   \star}\mathcal{M}:= \underline{\F^{\geq \star}M}\otimes_{\underline{\F^{\geq
    %\star}_\ev\THH(A;\bZ_p)}}\F^{\geq \star}_\ev\THH(\mathcal{O}_A;\bZ_p)\]
  %  and this will be the fully faithful left adjoint to the global sections functor. To see this it is enough to show that the above functor is in fact a sheaf. 

   % Let $A\to B$ be a quasisyntomic cover. It is enough to show that the map 
 %   \begin{align}\label{eqn: descent over thh}
  %      \F^{\geq \star}M\to \mathrm{Tot}(\bullet\mapsto\F^{\geq \star}M\otimes_{\F^{\geq
        %\star}_\ev\THH(A;\bZ_p)}\F^{\geq \star}_\ev\THH(B^{\otimes_A \bullet+1};\bZ_p))
    %\end{align} is an equivalence. We may also assume that each $B^{\otimes_A \bullet +1}$ is
    %quasiregular semiperfectoid by the unfolding equivalence, so that $\F^{\geq \star}_{\ev}\THH(B^{\otimes_A \bullet +1};\bZ_p)\simeq \tau_{\geq 2*}\THH(B^{\otimes_A \bullet +1};\bZ_p)$.
    %Since the forgetful functor to synthetic spectra is conservative we need only show that this map is an equivalence in synthetic spectra as well.

   % To this end let $\P$ be the Postnikov $t$-structure on synthetic spectra. Suppose now that
    %$\F^{\geq \star}M$ is bounded below. Then $\F^{\geq \star}M$ is also $u$-adically complete, where $u\in \pi_2\THH(R)=\pi_2(F^{\geq 1}_{\ev}\THH(R))$
   % is a generator of this group. Consequently we need only check that the map~\ref{eqn: descent over thh} is an equivalence modulo $u$,
   % where $\F^{\geq \star}_{\ev}\THH(A;\bZ_p)/u\simeq\F^{\geq
    %\star}_{\mathrm{HKR}}\mathrm{HH}(A/R)=\tau_{\geq\star}\mathrm{HH}(A/R)$ and $\F^{\geq
    %\star}_{\ev}\THH(B^{\otimes_A\bullet +1};\bZ_p)/u\simeq \tau_{\geq
    %2\star}\mathrm{HH}(B^{\otimes_A\bullet+1}/R)$. Thus it is enough to know that $\mathrm{HH}(A/R)\to
    %\mathrm{HH}(B/R)$ satisfies descent for modules, but this follows by the fact that $A\to B$ is
    %$p$-completely faithfully flat which is stable under taking tensor products.
    %For the general case, note that we have maps of fiber sequences 
    %\[
    %\begin{tikzcd}
    %    \tau_{\geq i}F^{\geq \star}M\ar[r] \ar[d] & \mathrm{Tot}(\bullet\mapsto (\tau_{\geq i}F^{\geq \star}M)\otimes_{F^{\geq \star}_\ev\THH(A;\bZ_p)}F^{\geq \star}_\ev\THH(B^{\otimes_A \bullet+1};\bZ_p))\ar[d]\\
     %   F^{\geq \star}M\ar[r] \ar[d] & \mathrm{Tot}(\bullet\mapsto F^{\geq \star}M\otimes_{F^{\geq \star}_\ev\THH(A;\bZ_p)}F^{\geq \star}_\ev\THH(B^{\otimes_A \bullet+1};\bZ_p))\ar[d]\\
      %  \tau_{\leq i-1}F^{\geq \star}M\ar[r] & \mathrm{Tot}(\bullet\mapsto (\tau_{\leq i-1}F^{\geq \star}M)\otimes_{F^{\geq \star}_\ev\THH(A;\bZ_p)}F^{\geq \star}_\ev\THH(B^{\otimes_A \bullet+1};\bZ_p))
    %\end{tikzcd}
    %\]
    %and the top horizontal map is an equivalence. Thus to finish the proof it is enough to see that the colimit as $i\to \infty$ of the bottom right corner term vanishes. Any bounded above $F^{\geq \star}_\ev\THH(R;\bZ_p)$-module is $u$-adically complete since on any given homotopy group multiplication by $u^N$ will be zero for $N$ large enough. Thus the same argument as in the bounded below case holds. 
%\end{proof}

%We will first compare the category $\CycSyn_{\F^{\geq \star}_\ev\THH(\mathcal{O}_A;\bZ_p)}$ to $F$-gauges for a general $A$,
%and then use this left adjoint to get a comparison in the smooth case.
%Before building this comparison, however, we will need a decompletion of all of the topological constructions consider thus far. 

%\begin{construction}
 %   \NR{Cite someone, not entirely sure who. I first saw this idea from Akhil, and then Rok convinced me it was correct.}
 %   Fix a base perfectiod ring $R$, and chose generators $u\in \pi_2(\F^{\geq 1}\THH(R;\bZ_p))$, a
 %   lift of $u$ to $\pi_2(\F^{\geq 1}(\F^{\geq \star}_\ev\THH(R;\bZ_p))^{\bT_{\ev}})$, and a
 %   generator $v\in \pi_{-2}(\F^{\geq -1}(\F^{\geq \star}_\ev\THH(R;\bZ_p))^{\bT_{\ev}})$. Let $\F^{\geq \star}M\in \SynSp_{\bT_{\ev},\F^{\geq \star}_\ev\THH(R;\bZ_p)}$. 
    
 %   Then we can define the decompleted filtered Tate construction of $\F^{\geq \star}M$ to be the
 %   filtered spectrum \[\mathrm{TP}_{dc}(\F^{\geq \star}M):= (\F^{\geq \star}M)^{\bT_{\ev}}[1/u],\]
 %   whose name is justified by the fact that if $A$ is a quasisyntomic $R$ algebra then
    %$\mathrm{gr}^i(\mathrm{TP}_{dc}(\F^{\geq \star}_\ev\THH(A;\bZ_p)))\simeq \prism_A\{i\}[2i]$. 
    
  %  Consider now $\F^{\geq \star}M$ a bounded below synthetic cyclotomic spectrum. In this case
  %  there is also a map \[\mathrm{TP}_{dc}(\F^{\geq \star}M)\to (\F^{\geq \star}M)^{t\bT_{\ev}}\]
  %  induced by the synthetic cyclotomic Frobenius on $\F^{\geq \star}M$.
  %  For such a map to exist it is enough to show that the synthetic cyclotomic Frobenius map
  %  $\phi_{\F^{\geq \star}M}^{\bT_\ev}\colon\F^{\geq \star}M^{\bT_\ev}\to (\F^{\geq \star}M^{tC_{p,\ev}})^{\bT_\ev}\simeq\F^{\geq \star}M^{t\bT_\ev}$ sends $u$ to an invertible element.
  %  This follows from the fact that $\phi_{\F^{\geq \star}M}^{\bT_{\ev}}$ is linear over the map
    %$\phi_{\F^{\geq\star}\THH(R;\bZ_p)}$ which sends $u$ to an invertible element. We may then define the decompleted fixed point construction as the pullback
   % \[
  %  \begin{tikzcd}
   %     \mathrm{TC}^-_{dc}(\F^{\geq \star}M) \ar[d] \ar[r] & (\F^{\geq \star}M)^{\bT_{\ev}}\ar[d,
  %      "\can"]\\
   %     \mathrm{TP}_{dc}(\F^{\geq \star}M)\ar[r] & (\F^{\geq \star}M)^{t\bT_\ev}
   % \end{tikzcd}
    %\]
    %and for $\F^{\geq \star}M=\F^{\geq \star}_\ev\THH(A;\bZ_p)$ we have that
    %$\mathrm{gr}^i\mathrm{TC}^{-}_{dc}(\F^{\geq \star}_\ev\THH(A:\bZ_p))\simeq \mathcal{N}^{\geq i}\prism_A\{i\}[2i]$.
   % Note that both of these constructions are functorial in $\F^{\geq \star}_\ev\THH(R;\bZ_p)$-modules,
   % and both constructions are independent of the choice of $R$, $u$, and $v$.
   % In particular this construction sheafifies to give functors \[\mathrm{TC}^{-}_{dc}(-),
  %  \mathrm{TP}_{dc}(-): \CycSyn_{\F^{\geq \star}_\ev\THH(\mathcal{O}_A;\bZ_p)}\to
  %  \SynSp_{\mathrm{TC}^-_{dc}(\F^{\geq \star}_\ev\THH(\mathcal{O}_A;\bZ_p))}\] for any quasisyntomic ring $A$. 
%\end{construction}

%\begin{construction}~\label{const: Gauge from Cycsyn}
   % We will first construct a functor $\mathrm{gr}^0_{\mathcal{N}^{\geq *}\prism}:\CycSyn_{\F^{\geq
    %\star}_\ev\THH(\mathcal{O}_R;\bZ_p)}\to
   % \mathcal{D}_{\mathrm{QCoh}}(\mathrm{Spf}(R)^{\mathcal{N}})$ such that
    %$\mathrm{gr}^0_\prism(\F^{\geq \star}_\ev\THH(\mathcal{O}_R;\bZ_p))\simeq
    %\mathrm{Fil}_N^*\mathcal{O}_{\prism}$. On quasiregular semiperfectoid rings this functor is
    %given by the $v$-adic filtration on $\mathrm{gr}^0\mathrm{TC}^{-}_{dc}(-)$. This is a Gauge by
   % \cite[Remark 5.5.4]{bhatt-fgauges}. More generally for $A$ a quasisyntomic ring, there is a
    %quasisyntomic cover $A\to S$ where $S$ is quasiregular semiperfectoid. In particular we have
    %that $\mathrm{Spf}(S)^\mathcal{N}\to \mathrm{Spf}(A)^\mathcal{N}$ is a flat surjection by
    %\cite[Remark 5.5.18]{bhatt-fgauges} and so to give a gauge on $A$ it is enough to give one on
    %$S$ together with descent data. In particular $\mathrm{gr}^0\mathrm{TC}^-_{dc}(-)$ with its
    %$v$-adic filtration gives a gauge as desired.
%\end{construction}

%\begin{construction}~\label{const: F-gauge from from Cycsyn}
  %  We will now construct a functor \[\mathrm{gr^0_{\textrm{F-Gauge}}}:\CycSyn_{\F^{\geq
    %\star}_{\ev}\THH(\mathcal{O}_R;\bZ_p)}\to
    %\mathcal{D}_{\mathrm{QCoh}}(\mathrm{Spf}(R)^{\mathrm{syn}})\] such that the underlying gauge is
    %that of Construction~\ref{const: Gauge from Cycsyn}. By definition giving an $F$-gauge is
    %equivalent to giving a prismatic gauge $\mathcal{M}$ on $\mathrm{Spf}(R)^\mathcal{N}$ together
    %with an identification $j_{HT}^*\mathcal{M}\simeq j_{dR}^*(\mathcal{M})$. Such data is given by
    %the functor considered in Construction~\ref{const: Gauge from Cycsyn} (for the gauge) together
    %with the map $\mathrm{gr}^0(\mathrm{TC}^-_{dc}(\F^{\geq
    %\star}\mathcal{M}(R))\xrightarrow{\phi_p}\mathrm{gr}^0(\mathrm{TP_{dc}(\F^{\geq
    %\star}\mathcal{M}(R))}))$ induced by the filtered Frobenius $\F^{\geq \star}\mathcal{M}\to
    %\F^{\geq \star}\mathcal{M}^{tC_{p,\ev}}$.
%\end{construction}



\subsection{\texorpdfstring{Lifts of Dieudonn{\'e} modules over smooth $\bF_p$-algebras}{Lifts of Dieudonn{\'e} modules over smooth algebras}}

Recall the following standard lemma.

\begin{lemma}~\label{lem: hearts and modules}
    Let $\mathcal{C}$ be a symmetric monoidal $\infty$-category, $\tau=(\mathcal{C}_{\geq
    0},\mathcal{C}_{\leq 0})$ a $t$-structure compatible with the monoidal structure, $R$ a
    connective $\bE_\infty$ ring, and $M$ and $N$ $\pi_0^\tau(R)$-modules in
    $\mathcal{C}^\heartsuit$. Then, the natural map $\mathrm{Maps}_R(M,N)\leftarrow
    \mathrm{Hom}_{\pi_0^\tau(R)}(M,N)$ is an equivalence.

\end{lemma}
% \begin{proof}
%     The space of maps $\mathrm{Maps}_{R}(M,N)$ is given by the totalization $\mathrm{Tot}(\bullet\mapsto \mathrm{Maps}_{\mathcal{C}}(M\otimes R^{\otimes \bullet},N))$. Each of the spaces in the totalization diagram are discrete since $M\otimes R^{\otimes \bullet}$ is connective and $N$ is coconnective, so therefore each of these mapping spaces are equivalent to $\mathrm{Hom}_{\mathcal{C}^\heartsuit}(M\otimes \pi_0^\tau(R)^{\otimes \bullet}, N)$, from which the result follows.
% \end{proof}

Now, let $A$ be a smooth $k$-algebra, $k$ a perfect $\bF_p$-algebra. Note that by
Remark~\ref{rem:bounds} $\F^{\geq \star}_{\ev}\THH(A;\bZ_p)$, and in fact $\F^{\geq
\star}_{\ev}\THH(R)$ for any $R\in \mathrm{CQSyn}$, will be connective in the Postnikov cyclotomic
$t$-structure. In particular by Lemma~\ref{lem: hearts and modules} the functor \[\pi_0^{\cyc,
\C}(\F^{\geq \star}_{\ev}\THH(A:\bZ_p))\mathrm{-Mod}(\CycSyn_p^\heartsuit)\hookrightarrow
\CycSyn_{\F^{\geq \star}_{\ev}\THH(A;\bZ_p)}\] induced by the ring map $\F^{\geq
\star}_\ev\THH(A;\bZ_p)\to \pi_0^{\tau^{Cyc}}(F^{\geq \star}_\ev\THH(A;\bZ_p))$ is fully faithful.
Thus in order to prove Theorem~\ref{thm: thmA} it is enough to show that formal p-divisible groups
over $A$ embed fully faithfully into the left hand category.

In order to do this we will need to identify the left hand category. Before stating the identification we will first recall some notation.

\begin{notation}
    For $A$ an $\bF_p$-algebra, denote by $W\Omega_A$ the de Rham Witt cochain complex of Illusie
    in \cite{illusie-derham-witt}. Denote by $W\Omega^{\geq i}_A$ the $i^{th}$ stage of the Hodge
    filtration.
\end{notation}

\begin{lemma}
    Let $A$ be a smooth algebra over a perfect $\bF_p$-algebra $k$. Then there is a natural
    identification \[\pi_i^{cyc, P}(\F^{\geq \star}_\ev\THH(A;\bZ_p))\cong W\Omega^{\geq i}_A\] in
    $\mathrm{DCart}^{\eta,\wedge}_V$, where the $F$, $V$, and $d$ maps are the usual ones, and
    $\eta=0$.
\end{lemma}
\begin{proof}
    The identification of $\CycSyn_p^\heartsuit\cong \mathrm{DCart}^{\eta, \wedge}_V$ goes through
    the t-exact functor $\mathrm{TR}:\CycSyn_p\to \syncart$, and so $\pi_i^{\cyc,\C}(\F^{\geq
    \star}_\ev\THH(A;\bZ_p))\cong \pi_i^{\tau^{Cart}}(\mathrm{TR}(\F^{\geq \star}_\ev
    \THH(A;\bZ_p)))$. The result then follows from \cite[Corollary 1.2]{Darrell_Riggenbach}.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm: thmA}]
    First recall that by \cite[Theorem 3.1]{DeJong_Messing_Deiudonne} the Deiudonn{\'e} functor
    $\mathbf{D}:\mathrm{FBT}_A^{op}\to C_A$ is fully faithful, where $C_S$ is the category of
    Deiudonn{\'e} crystals of finite presentation over $A$ together with an $F$ and $V$ operators,
    and lands in those crystals which are $V$-adically complete. Then \cite[Theorem
    1.1]{Bloch_Crystals} produces an embedding from $C_A\hookrightarrow
    W\Omega^*_A-\mathrm{Mod}(\mathrm{DCart}^\eta)$ which sends $V$-complete objects to $V$-complete
    objects. The result follows.
\end{proof}

\begin{conjecture}
    Let $A$ be a smooth $k$-algebra, $k$ a perfect $\bF_p$-algebra. Let \[\bD_{\CycSyn}:
    \mathrm{FBT}_A^{op}\hookrightarrow \CycSyn_{\F^{\geq \star}_\ev\THH(A;\bZ_p)}\] be the fully
    faithful embedding of Theorem~\ref{thm: thmA}. Then there is an equivalence
    \[\mathrm{gr}^0_{F-gauge}(\bD_\CycSyn)\simeq \bD_\prism\] where $\bD_\prism$ is the prismatic
    Dieudonn{\'e} functor of \cite{anschutz-lebras}.
\end{conjecture}

